Corpus Synthesis for Zero-shot ASR domain Adaptation using Large Language Models

While Automatic Speech Recognition (ASR) systems are widely used in many real-world applications, they often do not generalize well to new domains and need to be finetuned on data from these domains. However, target-domain data usually are not readily available in many scenarios. In this paper, we propose a new strategy for adapting ASR models to new target domains without any text or speech from those domains. To accomplish this, we propose a novel data synthesis pipeline that uses a Large Language Model (LLM) to generate a target domain text corpus, and a state-of-the-art controllable speech synthesis model to generate the corresponding speech. We propose a simple yet effective in-context instruction finetuning strategy to increase the effectiveness of LLM in generating text corpora for new domains. Experiments on the SLURP dataset show that the proposed method achieves an average relative word error rate improvement of $28\%$ on unseen target domains without any performance drop in source domains.

==> sections/backups/Method.tex <==
\section{Methodology}

\subsection{Problem Formulation}
Let $D_S$ denote as source domain data, $(X_S, Y_S, L_S) \in D_S$ denote as speech, corresponding text, and domain label in source domain. In this paper, we want to adapt ASR models $\theta^{S}$ trained on source domain $S$ to target domain $T$ without access to target domain $(X_T,  Y_T)$ but only access target domain label $L_T$.
\subsection{Data Synthesis Pipeline for ASR}
To accomplish domain adaptation with zero target domain resource, we propose a pipeline which using LLMs and TTS models to synthesize data.
Figure \ref{fig:framework} demonstrates the proposed pipeline, we first use $X_S, L_S$ as seed corpus for LLMs, and we use $L_T$ to extract $T$ related knowledge from LLMs. After we have synthesized TTS corpus, we then use well-trained TTS models to synthesize speech corpus for domain adaptation. In the ASR finetune stage, we add $Y_S$ as regularization to narrow the synthetic - real acoustic domain gap.
\subsection{LLM Generation}
In this section, we are going to describe two ways we utilize LLMs to prepare text corpus with $X_S$, $L_S$, and $L_T$.

\subsubsection{Instruction Finetuning}
To let synthesized texts has similar structures and styles to $X$, we employ the concept of instruction finetuning. As shown in Figure \ref{fig:example}, for each $x_s, l_s$, we first reformulate a instruction data "\textit{please generate a sentence related $l_s$: $x_s$}". With instruction finetuning, LLMs can learn the format and styles of source data $X_S$. When we provide a new label $l_t$, LLMs can generate similar fashion's sentences but correlated to target domain.

\subsubsection{In-Context Learning}
Another way to 
\begin{figure}[htp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/icl.pdf}
    \end{adjustbox}
    \caption{Example of demonstrations for ICL.}
    \label{fig:icl}
\end{figure}

==> sections/backups/Method2.tex <==
\section{Methodology}
\label{sec:method}
We provide an overview of our method in Fig. \ref{fig:framework}.
The overall pipeline consists of a large language model (LLM) a controllable speech synthesis (CSS) model and a pretrained ASR model.
%
Given a target domain of interest with domain name $d_t$, our goal is to generate a fully synthetic speech-text paired corpus $C_t={(x^t_i, y^t_i)}$, where $x^t_i$, $y^t_i$ are text content and speech signal of the $i-th$ sample, respectively.
%
To achieve this goal, we generate a text sentence $x^t_i \sim p_{LLM}(x | d_t)$ from the LLM conditioned on $d_t$, and then synthesize the corresponding $y^t_i \sim p_{CSS}(y|x_i)$ with the CSS model.
%
Then, we apply $C_t$ to perform ASR finetuning, and the finetuned ASR model shall receive better performance on the testing set of target domain.
%

Although preliminary experiment shows that naive usage of this pipeline already provides decent improvement, we find that it is important to address the discrepancy between real and synthetic text data distribution.
%
Considering that the LLM is trained on a very large-scale, general text corpus, it is difficult to produce high quality in-domain data with a target domain name $d_t$.
%
Thus, we further utilize a text corpus $C_s={(x^s_j, d^s_j)}$ derived from the training set of the pretrained ASR, where $d^s_j$ is the domain name of the $j-th$ sample.  
%
To this end, we propose a simple yet effective instruction finetuning strategy for LLM with $C_s$, and observe that it improves the quality of the synthetic text corpus.


\subsection{Large Language Model}
    % LLaMA 
 LLaMA \cite{touvron2023llama} is a state of the art foundation model that pretrained on 1.4T tokens with transformer-based architecture \cite{vaswani2017attention}. LLaMA-13B have shown to be able to outperforms GPT-3 (175B) \cite{brown2020language} on most benchmarks, and LLaMA- 65B is competitive with the best models, Chinchilla-70B \cite{hoffmann2022training} and PaLM-540B \cite{chowdhery2022palm}. In our experiments, we used LLaMA-7B \cite{touvron2023llama} to synthesize text data.

\subsection{Controllable Speech Synthesis (CSS) Model}
For CSS model, we adopt Style Equalization \cite{chang2022style}, which is designed based on Variational Recurrent Neural Net (VRNN) \cite{chung2015recurrent} and learns a prior distribution to model the acoustic style of speech.
%
By sampling from this prior distribution, the model can produce speech in various acoustic conditions.
%
To further enhance this capability, we make the following three simple modifications:
%
(1) increasing the number of gaussian mixtures of VRNN output distribution (from 3 to 10)
(2) enlarge the size of acoustic style feature (from 512 to 768)
(3) initialize the hidden states of VRNN using the average of the style vector sequence.
%
In this work, we train the modified Style Equalization model on the training set of LibriTTS \cite{zen2019libritts}.


\subsection{Instruction Finetuning (IF)}
\label{sec:instuct}
The concept of instruction finetuning is to formulate an natural language instruction with label and text, and use the formulate instruction to finetune LLMs. With instruction finetuning, LLMs has better ability to generalize to unseen data.


To make synthesized texts has similar format and styles to $C$, we apply the concept of instruction finetuning. As shown in Figure \ref{fig:example}, for each $x^s_j, d^s_j$, we first reformulate a instruction  \textit{"please generate a sentence related $d^s_j$: $x^s_j$"}. Secondly, we finetune LLM on the reformulated instruction data. The role of instruction here is to help LLMs better learn the format and styles of source text $x^s$, and the correlation between $d^s$ and $x^s$. 

When we provide a new label $d_t$, the instruct finetuned LLM can not only generate sentences with similar type to $C$, it can also related the label to the knowledge inside by instruction and make sentence fall into target domain.
\begin{table*}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{cccccccccccccccccccc}
\toprule
Zero-shot (WER)                                                   & \multicolumn{18}{c}{Testing Domains}                                                                                                                                                                                                                                                                                                     & \multirow{2}{*}{Average} \\ \cmidrule{1-19}
Methods                                                           & Alarm            & Audio            & Calendar         & Cooking          & Datetime         & Email            & General & IOT              & Lists            & Music           & News             & Play             & QA              & Recommendation   & Social           & Takeaway         & Transport        & Weather          &                          \\ \midrule
\begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular} & 8.0              & 13.1             & 12.8             & 18.2             & 11.2             & 19.0             & 14.4    & 19.2             & 14.6             & 10.5            & 15.3             & 24.8             & 22.3            & 15.7             & 26.3             & 26.5             & 17.1             & 12.9             & 16.77                    \\ \midrule
Instruction Finetuning                                            & \textbf{4.70}    & \textbf{8.17}    & \textbf{11.43}   & \textbf{11.90}   & \textbf{9.63}    & \textbf{14.43}   & 14.80   & \textbf{15.23}   & \textbf{11.30}   & \textbf{9.73}   & \textbf{12.83}   & \textbf{21.13}   & \textbf{20.90}  & \textbf{13.90}   & \textbf{19.43}   & \textbf{20.97}   & \textbf{10.73}   & \textbf{10.70}   & \textbf{13.44}           \\
WER Relative \%  $\uparrow$                                                 & \textbf{41.25\%} & \textbf{37.66\%} & \textbf{10.68\%} & \textbf{34.62\%} & \textbf{13.99\%} & \textbf{24.04\%} & -2.78\% & \textbf{20.66\%} & \textbf{22.60\%} & \textbf{7.30\%} & \textbf{16.12\%} & \textbf{14.78\%} & \textbf{6.28\%} & \textbf{11.46\%} & \textbf{26.11\%} & \textbf{20.88\%} & \textbf{37.23\%} & \textbf{17.05\%} & \textbf{19.86\%}         \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{ASR performance on Instruct Finetuned LLM.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
\label{tab:11000table}
\end{table*}

==> sections/backups/Method_old.tex <==
\section{Methodology}
\label{sec:method}
We provide an overview of the proposed approach in Fig.~\ref{fig:framework}.
The overall pipeline consists of an LLM, a CSS model, and a pretrained ASR model.
%
Given a target domain of interest, described using a word $d_t$, we first generate a fully synthetic text-speech paired corpus $C_t=\{(x^t_i, y^t_i)\}_{i=1}^N$, where $x^t_i$, $y^t_i$ are text content and speech signal of the $i$-th sample, respectively.
%
We do this by first generating a text sentence $x^t_i \sim p_{LLM}(x | d_t)$ from the LLM conditioned on $d_t$, and then synthesizing the corresponding speech $y^t_i \sim p_{CSS}(y|x_i^t)$ using the CSS model.
%
This synthetic data is finally used to adapt the ASR model to target domain $d_t$ by finetuning it. %, and the finetuned ASR model obtains better performance on the testing set of target domain.
%

% Although preliminary experiment shows that naive usage of this pipeline already provides decent improvement, we find that it is important to address the discrepancy between real and synthetic text data distribution.
% %
% Considering that the LLM is trained on a very large-scale, general text corpus, it is difficult to produce high quality in-domain data with a target domain name $d_t$.
% %
% Thus, we further utilize a text corpus $C_s={(x^s_j, d^s_j)}$ derived from the training set of the pretrained ASR, where $d^s_j$ is the domain name of the $j-th$ sample.  
% %
% To this end, we propose a simple yet effective instruction finetuning strategy for LLM with $C_s$, and observe that it improves the quality of the synthetic text corpus.


\subsection{Text Synthesis with LLMs}
    % LLaMA 
Given a target domain, our goal is to synthesize a text corpus that matches the target domain text distribution. For this, we utilize LLMs pretrained on trillions of text tokens by prompting them to generate sentences relavant for target domain. Specifically, we use the following prompt: \textit{Please generate a sentence related to $d_t$:}, where $d_t$ is the domain name.

While our experimental results show that leveraging the text corpus generated using off-the-shelf LLMs leads to some improvement in the final target domain ASR performance, the quality and relevance (to target domain) of generated text is not high.
%it is important to address the discrepancy between real and synthetic text data distribution.
Considering that off-the-shelf LLMs are trained on large-scale general text corpora, it is difficult for them to produce high quality in-domain data just based on the target domain name $d_t$.
% 
%To address this issue, we propose a simple yet effective instruction finetuning strategy that improves the ability of LLMs to generate in-domain data when prompted with the target domain name. 
To address this issue, we apply instruction finetuning and in-context learning to guide the decoding process of LLMs, improving their ability to generate in-domain data when prompted with the target domain name.
%constraint LLM generations and improve its generalizability toward unseen target domain.
 %Also, we further use a text corpus $C_s={(x^s_j, d^s_j)}$ derived from the training set of the pretrained ASR, where $d^s_j$ is the domain name of the $j$-th sample.  

\subsubsection{Instruction Finetuning (IF)}
\label{sec:instuct}
%\textbf{Instruction Finetuning (IF):}
The concept of instruction finetuning is to formulate a natural language instruction with a label and text, and use the formulated instruction to finetune LLMs. We use a text corpus $C_s={(x^s_j, d^s_j)}$ derived from the training set of the pretrained ASR, where $d^s_j$ is the domain name of the $j$-th sample.  
We use instruction finetuning to make the synthesized corpus have similar structure and styles to $C_s$. This enables the LLMs to generalize to unseen data.

%\todo{Fix notation in this paragraph, it is confusing.} 
%%%% Ting-Yao: we need to revisit this paragraph
As shown in Figure \ref{fig:example}, for each $x^s_j, d^s_j$, we first reformulate a instruction  \textit{"please generate a sentence related $d^s_j$: $x^s_j$"}. Secondly, we finetune the LLM on the reformulated instruction data. The role of instruction here is to help LLMs better learn the format and styles of the source text $x^s$, and the correlation between $d^s$ and $x^s$.

When we provide a new label $d_t$, the instruction finetuned LLM will not only generate sentences with similar structure to source corpora $C_s$, it also relates the label $d_t$ to its knowledge from pretraining
%the knowledge it learns from pretraining 
%\todo{better words to replace 'knowledge inside'} 
by instruction and generate text semantically related to the target domain.
%\begin{figure}[htp!]
\begin{figure}[tp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/new_example.pdf}
    \end{adjustbox}
    \caption{\textbf{Examples of instruction finetuning and zero-shot inferencing LLMs.} We explicitly relate domain name $d$ to text $x$ by reformulating an instruction to finetune LLMs. During inference, we use an unseen target domain with instruction to inference LLMs. }
    \label{fig:example}
\end{figure}
 % LLaMA \cite{touvron2023llama} is a state of the art foundation model that pretrained on 1.4T tokens with transformer-based architecture \cite{vaswani2017attention}. LLaMA-13B have shown to be able to outperforms GPT-3 (175B) \cite{brown2020language} on most benchmarks, and LLaMA- 65B is competitive with the best models, Chinchilla-70B \cite{hoffmann2022training} and PaLM-540B \cite{chowdhery2022palm}. In our experiments, we used LLaMA-7B \cite{touvron2023llama} to synthesize text data.

\subsubsection{In-context Learning (ICL)}
\label{sec:icl}
%\textbf{In-context Learning (ICL):}
In-context Learning is another way to steer pretrained LLMs' generation process. The mechanism of ICL is to provide some demonstrations for LLMs as examples and relies on LLMs' sentence completion ability to follow the examples and generate texts with similar format and styles. We provide ten demonstrations from the source domains for generation.
%\begin{figure}[htp!]
\begin{figure}[tp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/icl.pdf}
    \end{adjustbox}
    \caption{\textbf{Example of demonstrations for ICL.} We use the same instruction and iteratively randomly sample 10 demonstrations from source data to prompt LLMs.} %See \ref{sec:icl} for details. }
    \label{fig:icl}
\end{figure}
Figure \ref{fig:icl} is the constructed examples of ten demonstrations for pretrained LLaMA, we sampled ten sentences from source text $x^s$ as demonstrations for LLaMA iteratively until we get enough of text corpus.

\subsection{Speech Synthesis with Controllable Speech Synthesis (CSS) Model}
%After LLMs prepare a decent target domain text data, we employ a Controllable Speech Synthesis (CSS) Model to synthesize speech given text corpus $y^t_i \sim p_{CSS}(y|x_i)$.

We use the state-of-the-art Controllable Speech Synthesis CSS model \cite{chang2022style} to
synthesize speech $y^t_i \sim p_{CSS}(y|x^t_i)$, given the target domain text, $x^t_i$, generated by the instruction finetuned LLM model. 
%Different from the mainstream text-to-speech (TTS) models %\cite{shen2018natural,ren2020fastspeech},
The CSS model \cite{chang2022style} 
%To increase the acoustic diversity, we adopt Style Equalization \cite{chang2022style}, which is designed based on Variational Recurrent Neural Net (VRNN) \cite{chung2015recurrent} and 
learns a prior distribution to model the acoustic style of speech. By sampling from this prior distribution, the model can produce a synthetic speech corpus in various acoustic conditions.
%We use CSS model to synthesize various styles of speech $y^t_i \sim p_{CSS}(y|x_i)$ for downstream ASR finetuning.
% For CSS model, we adopt Style Equalization \cite{chang2022style}, which is designed based on Variational Recurrent Neural Net (VRNN) \cite{chung2015recurrent} and learns a prior distribution to model the acoustic style of speech.

\subsection{ASR Model Adaptation}
In the last step of our pipeline, we finetune the ASR model on the synthetic speech prepared by the LLM and CSS model. However, we observe that the ASR model usually over-fits to the synthetic speech artifacts during the finetuning stage, which limits the performance of the synthesis pipeline. 
%To address this problem, we add a small portion of the source domain real speech data along with the target domain synthesized speech data to regularize the ASR model's performance. 
To address this problem, we add the source domain real speech data along with the target domain synthesized speech data to regularize the ASR model's performance. 
%

%
% To further enhance this capability, we make the following three simple modifications:
% %
% (1) increasing the number of gaussian mixtures of VRNN output distribution (from 3 to 10)
% (2) enlarge the size of acoustic style feature (from 512 to 768)
% (3) initialize the hidden states of VRNN using the average of the style vector sequence.
% %
% In this work, we train the modified Style Equalization model on the training set of LibriTTS \cite{zen2019libritts}.





==> sections/backups/experimental_setups.tex <==
\section{Experimental Setups}
\subsection{Dataset}
%SLURP dataset \cite{bastianellietal2020slurp} is a spoken language understanding (SLU) dataset which consists of human's commands towards the robot, using 200 pre-defined prompts such as “How would you ask for the time.
%We split SLURP data according to 

SLURP dataset \cite{bastianellietal2020slurp} is a spoken language understanding (SLU) dataset which contains 16521 utterances of human’s commands towards a virtual agent, using 200 pre-defined prompts such as "How would you ask for the time.” 
%
The utterances are recorded in two types of acoustic environments (headset and far-field), and categorized into 18 domains (email, alarm, and takeaway, etc.). 

%[specify headset only]

In this work, we leverage the pre-defined 18 domains to form the experiment setup of zero-shot ASR domain adaptation.
%
Specifically, we combine 17 domains in SLURP to form the source domain, and use the rest one for target domain in testing phase.
%
Our method needs to improve the source domain ASR model without using any speech or text data of the target domain.
%
By conducting 18-fold cross validation, we report the word error rates (WERs) of the finetuned ASR models on the testing splits of 18 domains, respectively.



\subsection{ASR Model Adaptation}
We use ESPNet \cite{watanabe2018espnet} to build the end-to-end ASR model, which is composed of a conformer-based encoder \cite{gulati2020conformer} and a transformer-based decoder \cite{vaswani2017attention}.
%
In our experiment, we treat one domain in SLURP as the targete domain with zero-resrouce, and the combination of the rest 17 as the source domain real dataset. 
%
To obtain the source domain ASR model, we first pre-train the model on LibriSpeech \cite{panayotov2015librispeech}, and then finetune it on the source domain real dataset.
%
To adapt the source domain ASR model to the zero-resource target domain, we further finetune it on target domain synthetic dataset prepared by our method, along with a small portion of source domain real data (10\%).
%
We observe that it is important to include some real speech in the adaptation step, preventing the ASR model overfitting to the synthetic speech arctifact. 
%
The final checkpoint of source domain and finetuned ASR models are both selected according to their performance on target domain development set.


 \subsection{Baselines}
In this paper, we consider two generation methods to prompt directly, which are prompting pretrained LLMs directly with designed prompt and in-context learning LLM.
\subsubsection{Prompt Directly (PD) }
Recent works has shown that pretrained LLMs have good ability to complete the sentence by only providing a text in zero-shot fashion.
To adjust PD to our scenario, we directly prompt pretrained LLaMA by asking it \textit{'Please generate a sentence related to $d_t$:'} without providing any demonstrations from source data or training the LLaMA,
% However, since the style and format don't not match to the target domain data, we only gain limited improvements $4-22 \%$. 
\subsubsection{In-context Learning (ICL)}
 \label{sec:icl}
 In-context Learning is also considered another way to be used to steer pretrained LLMs' generation process. The mechanism of ICL is to provide some demonstrations for LLMs as examples and relies on LLMs' sentence completion ability to follow the examples and generate texts with similar format and styles.
  \begin{figure}[htp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/icl.pdf}
    \end{adjustbox}
    \caption{\textbf{Example of demonstrations for ICL.} We use the same instruction and iteratively randomly sample 10 demonstrations from source data to prompt LLMs. See \ref{sec:icl} for details. }
    \label{fig:icl}
\end{figure}
Figure \ref{fig:icl} is the constructed examples of ten demonstrations for pretrained LLaMA, we sampled ten sentence from source text $x^s$ as demonstrations for LLaMA iteratively under we get enough of text corpus. 




==> sections/backups/results.tex <==
\section{Results and Discussion}
% \begin{table}[!]
% \begin{adjustbox}{width=0.5\textwidth}

% \begin{tabular}{cccc}
% \toprule
% Word Error Rate (\%)                                                             & \multicolumn{3}{c}{Target Domains}                                        \\ \hline
% Methods                                                                     & Email                    & Alarm                   & Takeaway              \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular}           & 19.0                     & 8.0                     & 26.5                  \\ \midrule
% Prompt directly                                                             & 18.1 (7\%)               & 7.433 (4.7\%)           & 20.7 (21.9 \%)        \\ \midrule
% \multicolumn{1}{l}{In-Context Learning}                                     & \multicolumn{1}{l}{16.53 (12.98\%)}     & \multicolumn{1}{l}{5.77 (27.92 \%)}    & \multicolumn{1}{l}{22.07 (16.73\%)}  \\
% Instruction Finetuning                                                      & \textbf{15.43 (18.79\%)} & \textbf{4.43 (42.9 \%)} & \textbf{17.77 (33\%)} \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Real Text Only\\ (Access Real Text)\end{tabular} & 12.85                    & 5.375                   & 14.475                \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{ASR performance with different synthetic text data.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
%     \label{tab:11000table}
% \end{table}

\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}

\begin{tabular}{ccccccc}
\toprule
                             & SD ASR & PD & ICL    & IF & Real Text &  Real Speech \\ \midrule
WER $\downarrow$             & 16.77    & 16.24           & 16.23  & \textbf{13.44}         & 12.02                & 11.35           \\
(WER Relative \% $\uparrow$) & 0        & 3.169\%         & 3.21\% & \textbf{19.86\%}       & -                   & -              \\ \bottomrule
\end{tabular}

\end{adjustbox}
\caption{\textbf{ASR performance with different synthetic text data.} We take the average across domains and found that the corpus from instruct finetuned LLM perform the best. We compared source domain (SD) ASR with prompt directly (PD), in-context learning (ICL), and instruction finetuning (IF). We also report the ASR finetuned on real text synthetic speech (Real Text) and ASR finetuned with 18 domain real speech (Real Speech).
The metrics we use is WER (lower is better). }
\label{tab:method_compared}

\end{table}
\subsection{ASR Performance with Instruction Finetuned LLMs}
Table \ref{tab:11000table} shows the experiments results of ASR finetuned on the corpus synthesized with different methods. The results shown on Table \ref{tab:11000table} indicates that the ASR models finetuned on the corpus prepared from instruct finetuned LLMs gain huge improvements (average 19.86\%). The most we can achieve to 40\% relative improvement compared to the baseline. 
% \subsubsection{The Value of Instruction Finetuning}
By finetuning LLM on source domain data with instructions, we can explicitly relate domain name to texts. This results in the LLM having better generalizability towards unseen domain, and the generated synthetic corpus is closer to the target domain corpus $C_t$. 
We observe that the instruction finetuned LLM performance decreases for the \textit{'General'} domain. We attribute this as how specific the domain name is for the LLM. In this case, \textit{'Please generate a sentence related to general:'} is too vague and wide, so it's difficult for the LLM generated text to match to the target domain text without any examples from the target domain.
\subsection{What is the best Corpus Synthesis Strategy?}
Table \ref{tab:method_compared} shows the cross domain ASR average for the comparison between different LLM synthesize strategies. 

As shown in the Table \ref{tab:method_compared}, prompting pretrained LLaMA directly has shown little improvements from the baseline (3\% relative). After we demonstration some examples from source domain for pretrained LLaMA. The improvement is also limited (3\% relative) since it's difficult for the model to learn both the format from source domain and relate it to the target domain with just ten demonstrations each time.
Compared to the two baseline methods which leverage pretrained LLaMA, the instruction finetuned LLaMA can easily understand the format and style during supervised finetuning. It also shows that instruct-finetuned LLaMA has good generalizability to unseen domains. 
%\todo {not clear: help provoke potential knowledge in the pretraining stage}
\subsection{Quantitative Analysis of Synthetic Text}
\label{sec:quality}
We profile the generated text corpus as follows: 1) how close is the generated text to the real target domain and 2) the diversity of generated text corpus. We calculate the cosine similarity between synthetic text and real text of the target domain using the contextual embedding from Sentence-transformers\footnote{\url{https://www.sbert.net}, we use pretrained model-card \textit{'all-mpnet-base-v2'} to capture embedding.}. For measuring diversity, we use Self-BLEU 4 gram \cite{zhu2018texygen} and Distinct-1 and 2 \cite{li-etal-2016-diversity} to capture the corpus diversity and token repetitiveness.
%\todo {is `repeatness` the right word?}.
Table \ref{tab:quantitative} shows that although direct prompting and ICL can synthesize high diversity text, however they are not close to the real training set. On the other side, although the diversity of instruction finetuned LLaMA is lower, the generated text can improve target domain ASR performance the most since the generated corpus is close to the target domain text.
\begin{table}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccccc}
\toprule
                                                                 & D-1 $\uparrow$ & D-2$\uparrow$ & SB-4 $\downarrow$ & Similarity $\uparrow$ \\ \midrule
Test Set (Golden)                                                        &   0.49             &   0.867            & 0.276                  &   0.298                    \\ \midrule
Prompt Directly                                                  & 0.406          & 0.754         & 0.471             & 0.16                  \\
ICL                                                              & 0.589          & 0.841         & 0.424             & 0.18                  \\
\begin{tabular}[c]{@{}c@{}}Instruction Finetuning\end{tabular} & 0.488          & 0.869         & 0.74              & \textbf{0.245}        \\ \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{\textbf{Quantitative measurements of diversity and similarity towards target domain data.} We measure the synthetic text with Distinct 1 (D1) and 2 (D2), self-BLEU 4 (SB-4), and sentence cosine similarity.}
    \label{tab:quantitative}
\end{table}
\subsection{ASR Adaptation with Different Size of Text Corpus}

 \begin{figure}[htp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/transport.pdf}
    \end{adjustbox}
    \caption{\textbf{Number of synthetic text versus WER.} We measure the relationship between the number of synthetic text we used to finetune ASR and the corresponding WER. We verify this on domain \textit{'Transport'}. }
    \label{fig:tansport}
    
\end{figure}
Figure \ref{fig:tansport} shows the experiment results of using various amount of synthetic text to finetune ASR models and its corresponding WER. For instruction finetuned LLaMA, since the generations are close to target domain (Section \ref{sec:quality}), the WER continues to  go down when we increase the size of synthetic corpus  for ASR. 

%\todo{Don't understand the following sentence, are you referring to the baseline?}
% On the other hand, since the generation result from ICL is too far from target domain, we believe more synthetic text would be treated as noise for ASR models and the curve goes up when we increase the size of synthetic text using ICL. 
% \begin{table*}[]
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{cccccccccccccccccccc}
% \toprule
% Zero-shot (WER)                                                   & \multicolumn{18}{c}{Testing Domains}                                                                                                                                                                                                                                                                                                     & \multirow{2}{*}{Average} \\ \cmidrule{1-19}
% Methods                                                           & Alarm            & Audio            & Calendar         & Cooking          & Datetime         & Email            & General & IOT              & Lists            & Music           & News             & Play             & QA              & Recommendation   & Social           & Takeaway         & Transport        & Weather          &                          \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular} & 8.0              & 13.1             & 12.8             & 18.2             & 11.2             & 19.0             & 14.4    & 19.2             & 14.6             & 10.5            & 15.3             & 24.8             & 22.3            & 15.7             & 26.3             & 26.5             & 17.1             & 12.9             & 16.77                    \\ \midrule
% Instruction Finetuning                                            & \textbf{4.70}    & \textbf{8.17}    & \textbf{11.43}   & \textbf{11.90}   & \textbf{9.63}    & \textbf{14.43}   & 14.80   & \textbf{15.23}   & \textbf{11.30}   & \textbf{9.73}   & \textbf{12.83}   & \textbf{21.13}   & \textbf{20.90}  & \textbf{13.90}   & \textbf{19.43}   & \textbf{20.97}   & \textbf{10.73}   & \textbf{10.70}   & \textbf{13.44}           \\
% WER Relative \%  $\uparrow$                                                 & \textbf{41.25\%} & \textbf{37.66\%} & \textbf{10.68\%} & \textbf{34.62\%} & \textbf{13.99\%} & \textbf{24.04\%} & -2.78\% & \textbf{20.66\%} & \textbf{22.60\%} & \textbf{7.30\%} & \textbf{16.12\%} & \textbf{14.78\%} & \textbf{6.28\%} & \textbf{11.46\%} & \textbf{26.11\%} & \textbf{20.88\%} & \textbf{37.23\%} & \textbf{17.05\%} & \textbf{19.86\%}         \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{ASR performance on Instruct Finetuned LLM.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
% \label{tab:11000table}
% \end{table*}





% \begin{table}[]
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{ccccc}
% \toprule
%                                                                  & D-1 $\uparrow$ & D-2$\uparrow$ & SB-4 $\downarrow$ & Similarity $\uparrow$ \\ \midrule
% Test Set (Golden)                                                        &   0.49             &   0.867            & 0.276                  &   0.298                    \\ \midrule
% Prompt Directly                                                  & 0.406          & 0.754         & 0.471             & 0.16                  \\
% ICL                                                              & 0.589          & 0.841         & 0.424             & 0.18                  \\
% \begin{tabular}[c]{@{}c@{}}Instruction Finetuning\end{tabular} & 0.488          & 0.869         & 0.74              & \textbf{0.245}        \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
%     \caption{\textbf{Quantitative measurements of diversity and similarity towards target domain data.} We measure the synthetic text with Distinct 1 (D1) and 2 (D2), self-BLEU 4 (SB-4), and sentence cosine similarity.}
%     \label{tab:quantitative}
% \end{table}

==> sections/backups/results_old.tex <==
\section{Results and Discussion}

\begin{table*}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{cccccccccccccccccccc}
\toprule
Zero-shot (WER)                                                   & \multicolumn{18}{c}{Testing Domains}                                                                                                                                                                                                                                                                                                                & \multirow{2}{*}{Average} \\ \cmidrule{1-19}
Methods                                                           & Alarm            & Audio            & Calendar         & Cooking          & Datetime         & Email            & General          & IOT              & Lists            & Music            & News             & Play             & QA               & Recommendation   & Social           & Takeaway         & Transport        & Weather          &                          \\ \midrule
\begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular} & 8.0              & 13.1             & 12.8             & 18.2             & 11.2             & 19.0             & 14.4             & 19.2             & 14.6             & 10.5             & 15.3             & 24.8             & 22.3             & 15.7             & 26.3             & 26.5             & 17.1             & 12.9             & 16.77                    \\ \midrule
In-context Learning                                               & \textbf{5.97}    & \textbf{7.40}    & \textbf{10.47}   & \textbf{10.07}   & \textbf{8.03}    & \textbf{13.37}   & \textbf{12.57}   & \textbf{8.93}    & \textbf{11.10}   & \textbf{8.73}    & \textbf{10.33}   & \textbf{20.90}   & \textbf{21.50}  & \textbf{13.80}   & \textbf{17.23}   & \textbf{19.10}   & \textbf{9.93}    & \textbf{8.93}    & \textbf{12.13}           \\
WER Relative \%                                                   & \textbf{25.42\%} & \textbf{43.51\%} & \textbf{18.23\%} & \textbf{44.69\%} & \textbf{28.27\%} & \textbf{29.65\%} & \textbf{12.73\%} & \textbf{53.47\%} & \textbf{23.97\%} & \textbf{16.83\%} & \textbf{32.46\%} & \textbf{15.73\%} & \textbf{3.59\%} & \textbf{12.10\%} & \textbf{34.47\%} & \textbf{27.92\%} & \textbf{41.91\%} & \textbf{30.75\%} & \textbf{27.67\%}      \\ \bottomrule

% Instruction Finetuning                                            & \textbf{4.70}    & \textbf{8.17}    & \textbf{11.43}   & \textbf{11.90}   & \textbf{9.63}    & \textbf{14.43}   & 14.80   & \textbf{15.23}   & \textbf{11.30}   & \textbf{9.73}   & \textbf{12.83}   & \textbf{21.13}   & \textbf{20.90}  & \textbf{13.90}   & \textbf{19.43}   & \textbf{20.97}   & \textbf{10.73}   & \textbf{10.70}   & \textbf{13.44}           \\
% %WER Relative \%  $\uparrow$                                                 & \textbf{41.25\%} & \textbf{37.66\%} & \textbf{10.68\%} & \textbf{34.62\%} & \textbf{13.99\%} & \textbf{24.04\%} & -2.78\% & \textbf{20.66\%} & \textbf{22.60\%} & \textbf{7.30\%} & \textbf{16.12\%} & \textbf{14.78\%} & \textbf{6.28\%} & \textbf{11.46\%} & \textbf{26.11\%} & \textbf{20.88\%} & \textbf{37.23\%} & \textbf{17.05\%} & \textbf{19.86\%}         \\ \bottomrule
% Relative WER Reduction\%  $\uparrow$                                                 & \textbf{41.25} & \textbf{37.66} & \textbf{10.68} & \textbf{34.62} & \textbf{13.99} & \textbf{24.04} & -2.78 & \textbf{20.66} & \textbf{22.60} & \textbf{7.30} & \textbf{16.12} & \textbf{14.78} & \textbf{6.28} & \textbf{11.46} & \textbf{26.11} & \textbf{20.88} & \textbf{37.23} & \textbf{17.05} & \textbf{19.86}         \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{ASR performance on Instruct Finetuned LLM.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
\label{tab:11000table}
\end{table*}

% \begin{table}[!]
% \begin{adjustbox}{width=0.5\textwidth}

% \begin{tabular}{cccc}
% \toprule
% Word Error Rate (\%)                                                             & \multicolumn{3}{c}{Target Domains}                                        \\ \hline
% Methods                                                                     & Email                    & Alarm                   & Takeaway              \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular}           & 19.0                     & 8.0                     & 26.5                  \\ \midrule
% Prompt directly                                                             & 18.1 (7\%)               & 7.433 (4.7\%)           & 20.7 (21.9 \%)        \\ \midrule
% \multicolumn{1}{l}{In-Context Learning}                                     & \multicolumn{1}{l}{16.53 (12.98\%)}     & \multicolumn{1}{l}{5.77 (27.92 \%)}    & \multicolumn{1}{l}{22.07 (16.73\%)}  \\
% Instruction Finetuning                                                      & \textbf{15.43 (18.79\%)} & \textbf{4.43 (42.9 \%)} & \textbf{17.77 (33\%)} \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Real Text Only\\ (Access Real Text)\end{tabular} & 12.85                    & 5.375                   & 14.475                \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{ASR performance with different synthetic text data.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
%     \label{tab:11000table}
% \end{table}

\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}

\begin{tabular}{ccccccc}
\toprule
                             & SD ASR & PD & IF    & \textbf{ICL} & Real Text &  Real Speech \\ \midrule
WER $\downarrow$             & 16.77    & 14.02           & 12.59  & \textbf{12.13}         & 12.02                & 11.35           \\
Relative WER Reduction\% $\uparrow$ & -        & 16.40         & 24.92 & \textbf{27.67}       & -                   & -              \\ \bottomrule
\end{tabular}

\end{adjustbox}
\caption{\textbf{ASR performance with different synthetic text data.} We take the average across domains and found that the corpus from instruct finetuned LLM perform the best. We compared source domain (SD) ASR with prompt directly (PD), in-context learning (ICL), and instruction finetuning (IF). We also report the ASR finetuned on real text synthetic speech (Real Text) and ASR finetuned with 18 domain real speech (Real Speech).
The metrics we use is WER (lower is better). }
\label{tab:method_compared}

\end{table}

\subsection{ASR Performance with Instruction Finetuned LLMs}
Table \ref{tab:11000table} shows the experimental results of ASR finetuned on the corpus synthesized with different methods. The results shown on Table \ref{tab:11000table} indicates that the ASR models finetuned on the corpus prepared from instruction finetuned LLaMA gain large improvements (average 22.19\%). The most we can achieve to 40\% relative improvement compared to the baseline. 
% \subsubsection{The Value of Instruction Finetuning}
By finetuning the LLM on source domain data with instructions, we can explicitly relate domain name to texts.
%% Ting-Yao: need revisit
The results indicate the LLM having better generalizability towards an unseen domain, and the generated synthetic corpus being closer to the target domain. 
% We observe that the instruction finetuned LLM performance decreases for the \textit{'General'} domain. We attribute this as how specific the domain name is for the LLM. In this case, \textit{'Please generate a sentence related to general:'} is too vague, so it is difficult for the LLM to generate text to match to the target domain text without any examples from the target domain.

\subsection{What is the best Corpus Synthesis Strategy?}
Table \ref{tab:method_compared} shows the cross domain ASR average for the comparison between different LLM synthesis strategies. 

As shown in the Table \ref{tab:method_compared}, prompting pretrained LLaMA directly has shown little improvements from the baseline (3\% relative). After  demonstrating some examples from the source domain for pretrained LLaMA, the improvement is also limited (3\% relative) since it is difficult for the model to learn both the format from the source domain and relate it to the target domain with just 10 demonstrations. % each time.
Compared to the two baseline methods which use pretrained LLaMA, the instruction finetuned LLaMA can easily understand the format and style. %during supervised finetuning. 
It also shows that instruct-finetuned LLaMA has good generalizability to unseen domains. 
%\todo {not clear: help provoke potential knowledge in the pretraining stage}
\subsection{Quantitative Analysis of Synthetic Text}
\label{sec:quality}
We profile the generated text corpus as follows: 1) how close is the generated text to the real target domain and 2) the diversity of generated text corpus. %We calculate the Jesen-Shannon divergence between synthetic text token distribution and real text of the target domain token distribution to measure the similarity \cite{ruder2017data}.
We calculate the Jesen-Shannon divergence between synthetic and real text token distributions to measure the similarity \cite{ruder2017data}.
For measuring diversity, we use Self-BLEU 4 gram \cite{zhu2018texygen} and Distinct-1 and 2 \cite{li-etal-2016-diversity} to capture the corpus diversity and token repetitiveness.
%\todo {is `repeatness` the right word?}.
Table \ref{tab:quantitative} shows that although direct prompting and ICL can synthesize high diversity text, they are not close to the real training set. On the other side, although the diversity of instruction finetuned LLaMA is lower, the generated text can improve target domain ASR performance the most since the generated corpus is close to the target domain text.
\begin{table}[]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{ccccc}
\toprule
                                                                 & D-1 $\uparrow$ & D-2$\uparrow$ & SB-4 $\downarrow$ & JS-Div $\downarrow$ \\ \midrule
Test Set (Golden)                                                        &   0.49             &   0.867            & 0.276                  &   0.43                    \\ \midrule
Prompt Directly                                                  & 0.406          & 0.754         & 0.471             & 0.521                  \\
ICL                                                              & 0.589          & 0.841         & 0.424             & 0.482                  \\
\begin{tabular}[c]{@{}c@{}}Instruction Finetuning\end{tabular} & 0.488          & 0.869         & 0.74              & \textbf{0.451}        \\ \bottomrule
\end{tabular}
\end{adjustbox}
    \caption{\textbf{Quantitative measurements of synthetic corpus in terms of diversity and similarity towards target domain real data.} We measure the synthetic text with Distinct 1 (D1) and 2 (D2), self-BLEU 4 (SB-4), and Jensen-Shannon divergence (JS-Div).}
    \label{tab:quantitative}
\end{table}

%\iffalse
\subsection{ASR Adaptation with Different Size of Text Corpus}

 \begin{figure}[htp!]
    \begin{adjustbox}{width=\linewidth}
    \centering
    \includegraphics{pics/transport.pdf}
    \end{adjustbox}
    \caption{\textbf{Number of synthetic text versus WER.} We measure the relationship between the number of synthetic text we used to finetune ASR and the corresponding WER. We verify this on domain \textit{'Transport'} and \textit{'Cooking'}. }
    \label{fig:tansport}
    
\end{figure}
Figure \ref{fig:tansport} shows the experimental results from using various amount of synthetic text to finetune ASR models, and its corresponding WER. 
%% Ting-Yao: need to be revisited
In the figure, the x axis is the number of synthetic text used to finetune ASR model and the y axis is the absolute WER. We plot the figures on \textit{'Transport'} and \textit{'Cooking'} Domain.
In the figure, we can observe that when we use more synthetic data to finetune ASR model, the increased text diversity make the performance keeps going up. On the other side, we can also observe ASR performance saturated on 55k synthetic data, we believe it's because there are some synthetic artifact as noise that decrease the performance. We leave this as a furture work to eliminate outliers from synthetic data.
% For instruction finetuned LLaMA, since the generations are close to target domain (Section \ref{sec:quality}), the WER continues to decrease when we increase the size of synthetic corpus  for ASR. 
%\fi
%\todo{Don't understand the following sentence, are you referring to the baseline?}
% On the other hand, since the generation result from ICL is too far from target domain, we believe more synthetic text would be treated as noise for ASR models and the curve goes up when we increase the size of synthetic text using ICL. 
% \begin{table*}[]
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{cccccccccccccccccccc}
% \toprule
% Zero-shot (WER)                                                   & \multicolumn{18}{c}{Testing Domains}                                                                                                                                                                                                                                                                                                     & \multirow{2}{*}{Average} \\ \cmidrule{1-19}
% Methods                                                           & Alarm            & Audio            & Calendar         & Cooking          & Datetime         & Email            & General & IOT              & Lists            & Music           & News             & Play             & QA              & Recommendation   & Social           & Takeaway         & Transport        & Weather          &                          \\ \midrule
% \begin{tabular}[c]{@{}c@{}}Original ASR\\ (Baseline)\end{tabular} & 8.0              & 13.1             & 12.8             & 18.2             & 11.2             & 19.0             & 14.4    & 19.2             & 14.6             & 10.5            & 15.3             & 24.8             & 22.3            & 15.7             & 26.3             & 26.5             & 17.1             & 12.9             & 16.77                    \\ \midrule
% Instruction Finetuning                                            & \textbf{4.70}    & \textbf{8.17}    & \textbf{11.43}   & \textbf{11.90}   & \textbf{9.63}    & \textbf{14.43}   & 14.80   & \textbf{15.23}   & \textbf{11.30}   & \textbf{9.73}   & \textbf{12.83}   & \textbf{21.13}   & \textbf{20.90}  & \textbf{13.90}   & \textbf{19.43}   & \textbf{20.97}   & \textbf{10.73}   & \textbf{10.70}   & \textbf{13.44}           \\
% WER Relative \%  $\uparrow$                                                 & \textbf{41.25\%} & \textbf{37.66\%} & \textbf{10.68\%} & \textbf{34.62\%} & \textbf{13.99\%} & \textbf{24.04\%} & -2.78\% & \textbf{20.66\%} & \textbf{22.60\%} & \textbf{7.30\%} & \textbf{16.12\%} & \textbf{14.78\%} & \textbf{6.28\%} & \textbf{11.46\%} & \textbf{26.11\%} & \textbf{20.88\%} & \textbf{37.23\%} & \textbf{17.05\%} & \textbf{19.86\%}         \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{ASR performance on Instruct Finetuned LLM.} The LLMs with instruction finetuned synthesize the text corpus to finetune ASR models. The metrics we use is WER (lower is better). } 
% \label{tab:11000table}
% \end{table*}





% \begin{table}[]
% \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{ccccc}
% \toprule
%                                                                  & D-1 $\uparrow$ & D-2$\uparrow$ & SB-4 $\downarrow$ & Similarity $\uparrow$ \\ \midrule
% Test Set (Golden)                                                        &   0.49             &   0.867            & 0.276                  &   0.298                    \\ \midrule
% Prompt Directly                                                  & 0.406          & 0.754         & 0.471             & 0.16                  \\
% ICL                                                              & 0.589          & 0.841         & 0.424             & 0.18                  \\
% \begin{tabular}[c]{@{}c@{}}Instruction Finetuning\end{tabular} & 0.488          & 0.869         & 0.74              & \textbf{0.245}        \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
%     \caption{\textbf{Quantitative measurements of diversity and similarity towards target domain data.} We measure the synthetic text with Distinct 1 (D1) and 2 (D2), self-BLEU 4 (SB-4), and sentence cosine similarity.}
%     \label{tab:quantitative}
% \end{table}
